Dyadic Human Motion Prediction

Prior work on human motion forecasting has mostly focused on predicting the future motion of single subjects in isolation from their past pose sequence. In the presence of closely interacting people, however, this strategy fails to account for the dependencies between the different subject's motions. In this paper, we therefore introduce a motion prediction framework that explicitly reasons about the interactions of two observed subjects. Specifically, we achieve this by introducing a pairwise attention mechanism that models the mutual dependencies in the motion history of the two subjects. This allows us to preserve the long-term motion dynamics in a more realistic way and more robustly predict unusual and fast-paced movements, such as the ones occurring in a dance scenario. To evaluate this, and because no existing motion prediction datasets depict two closely-interacting subjects, we introduce the LindyHop600K dance dataset. Our results evidence that our approach outperforms the state-of-the-art single person motion prediction techniques.

==> figures/lhop_qualitative_follower.tex <==
\begin{figure*}
	\vspace{-4mm}
	\centering
	\begin{tabular}{c}
		\includegraphics[width=1.0\linewidth]{figures/qualitative_lhop_sota.pdf} \\
	\end{tabular}
	\vspace{-3mm}
	\caption[Qualitative 3D motion prediction results on the \lindyhop{} test subject with the follower role]{\textbf{Qualitative evaluation of our results on the \lindyhop{} test subject with the follower role compared to the state-of-the-art methods.} Black: Ground truth, green: TIM~\cite{Lebailly20}, blue: MSR-GCN~\cite{Lingwei21}, violet: HRI~\cite{Mao20}, red: Ours-Dyadic. The left side of the vertical bar in the black row depicts the sampled input to our model and the right side shows the ground truth future poses. The colored rows correspond to the predictions of the state-of-the-art single person approaches. The red row depicts the output of our model shown in Fig.~\ref{fig:overview_3dmotion_forecasting}. The numbers at the top indicate the future timestamp in milliseconds.}
	\label{fig:qualitative_lhop_sota}
\end{figure*}


==> figures/lhop_qualitative_leader.tex <==
\begin{figure*}
	\vspace{-4mm}
	\centering
	\begin{tabular}{c}
		\includegraphics[width=1.0\linewidth]{figures/qualitative_lhop_sota2.pdf} \\
	\end{tabular}
	\vspace{-3mm}
	\caption[Qualitative 3D motion prediction results on the \lindyhop{} test subject with the leader role]{\textbf{Qualitative evaluation of our results on the \lindyhop{} test subject with the leader role compared to the state-of-the-art methods.} Black: Ground truth, green: TIM~\cite{Lebailly20}, blue: MSR-GCN~\cite{Lingwei21}, violet: HRI~\cite{Mao20}, red: Ours-Dyadic. The left side of the vertical bar in the black row depicts the sampled input to our model and the right side shows the ground truth future poses. The colored rows correspond to the predictions of the state-of-the-art single person approaches. The red row depicts the output of our model shown in Fig.~\ref{fig:overview_3dmotion_forecasting}. The numbers at the top indicate the future timestamp in milliseconds.}
	\label{fig:qualitative_lhop_sota_2}
\end{figure*}
